Robust Distributed Arrays: Provably Secure Networking for Data Availability Sampling

Data Availability Sampling (DAS), a central component of Ethereum's roadmap, enables clients to verify data availability without requiring any single client to download the entire dataset. DAS operates by having clients randomly retrieve individual symbols of erasure-encoded data from a peer-to-peer network. While the cryptographic and encoding aspects of DAS have recently undergone formal analysis, the peer-to-peer networking layer remains underexplored, with a lack of security definitions and efficient, provably secure constructions. In this work, we address this gap by introducing a novel distributed data structure that can serve as the networking layer for DAS, which we call robust distributed arrays. That is, we rigorously define a robustness property of a distributed data structure in an open permissionless network, that mimics a collection of arrays. Then, we give a simple and efficient construction and formally prove its robustness. Notably, every individual node is required to store only small portions of the data, and accessing array positions incurs minimal latency. The robustness of our construction relies solely on the presence of a minimal absolute number of honest nodes in the network. In particular, we avoid any honest majority assumption. Beyond DAS, we anticipate that robust distributed arrays can have wider applications in distributed systems.

==> additional.tex <==
\ifnum\submission=1
	\usepackage[pdfpagelabels=true,linktocpage=true,colorlinks=true]{hyperref}
\else
	\usepackage[pdfpagelabels=true,linktocpage=true,pagebackref,colorlinks=true]{hyperref}
	\ifnum\llncs=0
		\renewcommand*{\backref}[1]{(Cited on Page~#1.)}
	\fi
\fi % If submission=1: pagebackrefs are deactivated
	% If submission=0 and not using lncs `Cited on page...' is added to each entry in hte biblio

% ---------------------------------------------------------------------
\def\titleofpdf{\titletext}		%automatically embeds the title into pdf info. Part 1
\def\authorsofpdf{%				%automatically embeds the author names your pdf info. Part 1
\ifcsname 5name\endcsname
	\csname 1name\endcsname~et~al.
\else
	\ifcsname 1name\endcsname
		\csname 1name\endcsname
		\ifcsname 3name\endcsname
			,\ \csname 2name\endcsname
			\ifcsname 4name\endcsname
				,\ \csname 3name\endcsname\ and \csname 4name\endcsname
			\else%
				\ and\ \csname 3name\endcsname
			\fi
		\else
			\ifcsname 2name\endcsname
				\csname 2name\endcsname
			\fi
		\fi
	\fi
\fi
}

\ifnum\submission=1 %link colours are set to black when submission=1
	\hypersetup{
	pdftitle={\titleofpdf}, %embedding of title into pdf info. Part 2
	pdfauthor=\ifnum\anonymous=0{\authorsofpdf}\else{}\fi, %author pdf info embed. when not anonym.
	linkcolor=[rgb]{0,0,0}, %link colours are set to black.
	urlcolor=[rgb]{0,0,0},  %link colours are set to black.
	citecolor=[rgb]{0,0,0}  %link colours are set to black.
	}
\else
	\hypersetup{
	pdftitle={\titleofpdf},
	pdfauthor=\ifnum\anonymous=0{\authorsofpdf}\else{}\fi,
	linkcolor=[rgb]{0,0,0.5},
	urlcolor=[rgb]{0,0,0.5},
	citecolor=[rgb]{0,0,0.5}
	}
\fi
% ---------------------------------------------------------------------

%load cleveref always after hyperref
\ifnum\abbrevref=0
	\usepackage[capitalise,noabbrev]{cleveref}
\else
	\usepackage[capitalise]{cleveref}
\fi

\usepackage{nicodemus}
\usepackage[absolute]{textpos}	% used for warning messages and publication info
\usepackage{everypage}			% used for the page limit warning



\ifnum\LNCSpreview=1 %LNCS review reminder watermark
	\usepackage[paperwidth=152mm,paperheight=235mm,textwidth=122mm,textheight=193mm]{geometry}
	\AddEverypageHook{
		\begin{textblock}{1}[1,1](0.5,0.9)
			\centering\Large
			\textcolor{lightgray}{\textbf{LNCS Preview mode active.}}
		\end{textblock}
	}
	\def\choosepubinfo{0}
\fi

\ifnum\overflow=1
	\overfullrule=2mm
\fi

\ifnum\allowbreaks=1
	\allowdisplaybreaks
\fi

\ifnum\showlabels=1
	\usepackage{showkeys}
\fi

\ifnum\submission=1
	\def\authnotes{0}
\fi

\ifnum\anonymous=1
	\def\authnotes{0}
\fi

\ifx\pagelimit\empty %page limit warning magic
\else
	\newcounter{pagewarning}
	\setcounter{pagewarning}{\pagelimit}
	\AddEverypageHook{
		\ifnum\thepage>\thepagewarning
			\ifnum\LNCSpreview=0
				\begin{textblock}{1}[0.5,0](0,-13.5)
			\else
				\begin{textblock}{1}[0.5,0](0,-11.95)
			\fi
				\centering\Large
				\textcolor{red}{\textbf{This page is exceeding the page limit.}}
			\end{textblock}
		\fi
}
\fi

\def\notesindocument{0}

\newlength{\strutdepth}%
\settodepth{\strutdepth}{\strutbox}%

\newcommand{\notes}[3]{ %framework for margin notes of any kind
\ifnum\authnotes=1
	\def\notesindocument{1}%
	\noindent{%\bfseries
	\color{#1}{#3}\color{#1}}%
	\strut\vadjust{\kern-\strutdepth%
		\vtop to \strutdepth{%
			\baselineskip\strutdepth%
			\vss\llap{{\large\color{#1}\textbf{#2}\quad\color{black}}}\null%
		}%
	}%
\fi
}

% below you see how to set up margin notes. hspace hack for using paper size cropped to lncs size
\ifnum\LNCSpreview=0
	\newcommand{\todo}[1]{\notes{Red}{TODO}{#1}}
	\newcommand{\new}[1]{\notes{ForestGreen}{NEW}{#1}}
	\newcommand{\alert}[1]{\notes{Red}{ALERT}{#1}}
	\newcommand{\authornote}[1]{\notes{black}{NOTE}{#1}}
\else
	\newcommand{\todo}[1]{\notes{Red}{Todo\hspace{-1.5ex}}{#1}}
	\newcommand{\new}[1]{\notes{ForestGreen}{New\hspace{-1.5ex}}{#1}}
	\newcommand{\alert}[1]{\notes{Red}{Alert\hspace{-1.5ex}}{#1}}
	\newcommand{\authornote}[1]{\notes{black}{Note\hspace{-1.5ex}}{#1}}
\fi

\newcommand{\authnote}[2]{ %command for authnotes that appear in the text body
	\ifnum\authnotes=1
		\def\notesindocument{1}
		\begin{center}
			\fbox{%
				\begin{minipage}{.98\textwidth}
					\textbf{#1 says:} #2\authornote{}
				\end{minipage}%
			}
		\end{center}
	\fi
}

\ifnum\llncs=1
	\ifnum\llncsqedsymbol=1
		\let\oldproof\proof
		\renewenvironment{proof}%
		{\begin{oldproof}}%
		{\qed\end{oldproof}}
	\fi
\fi

%
\ifnum\llncs=0				%definition of new environemnt styles when not using llncs
\usepackage{newpxtext} %\usepackage[euler-digits]{eulervm}

\newtheoremstyle{mytheorem}
  {\topsep} % Space above
  {\topsep} % Space below
  {} % Body font
  {} % Indent amount
  {\bfseries} % Theorem head font
  {} % Punctuation after theorem head
  {.5em} % Space after theorem head
  {\thmname{#1}\thmnumber{ #2}\thmnote{ {\bfseries (#3)}}.} % Theorem head spec

\newtheoremstyle{myplain}
  {\topsep} % Space above
  {\topsep} % Space below
  {\itshape} % Body font
  {} % Indent amount
  {\bfseries} % Theorem head font
  {} % Punctuation after theorem head
  {.5em} % Space after theorem head
  {\thmname{#1}\thmnumber{ #2}\thmnote{ {\normalfont(#3)}}.} % Theorem head spec

\newtheoremstyle{mydefinition}
  {\topsep} % Space above
  {\topsep} % Space below
  {} % Body font
  {} % Indent amount
  {\bfseries} % Theorem head font
  {} % Punctuation after theorem head
  {.5em} % Space after theorem head
  {\thmname{#1}\thmnumber{ #2}\thmnote{ {\normalfont(#3)}}.} % Theorem head spec

\newtheoremstyle{myremark}
  {} % Space above
  {} % Space below
  {} % Body font
  {} % Indent amount
  {\itshape} % Theorem head font
  {} % Punctuation after theorem head
  {.5em} % Space after theorem head
  {\thmname{#1}\thmnumber{ #2}\thmnote{ {\normalfont(#3)}}.} % Theorem head spec

	\theoremstyle{mytheorem}				% new theorem-like environments when llncs=0
	\newtheorem{theorem}{Theorem}

	\theoremstyle{myplain}
	\newtheorem{lemma}{Lemma}
	\newtheorem{corollary}{Corollary}
	\newtheorem{proposition}{Proposition}
	\newtheorem{construction}{Construction}
	\newtheorem{conjecture}{Conjecture}

	\theoremstyle{mydefinition}
	\newtheorem{definition}{Definition}
	\newtheorem{claim}{Claim}
	\newtheorem{assumption}{Assumption}
	\newtheorem{fact}{Fact}

	\theoremstyle{myremark}
	\newtheorem{remark}{Remark}
	\newtheorem{example}{Example}
	\newtheorem{note}{Note}
	\newtheorem{observation}{Observation}
\else									% new theorem-like environments when llncs=1
	\spnewtheorem{construction}[theorem]{Construction}{\bfseries}{}
	\spnewtheorem{assumption}[theorem]{}{\bfseries}{}
	\spnewtheorem{fact}[theorem]{Fact}{\bfseries}{}

	\spnewtheorem{observation}[theorem]{Observation}{\itshape}{}
\fi

% to save some typing
\newenvironment{theo}{\begin{theorem}}{\end{theorem}}
\newenvironment{thm}{\begin{theorem}}{\end{theorem}}
\newenvironment{lemm}{\begin{lemma}}{\end{lemma}}
\newenvironment{lem}{\begin{lemma}}{\end{lemma}}
\newenvironment{coro}{\begin{corollary}}{\end{corollary}}
\newenvironment{cor}{\begin{corollary}}{\end{corollary}}
\newenvironment{prop}{\begin{proposition}}{\end{proposition}}
\newenvironment{conj}{\begin{conjecture}}{\end{conjecture}}
\newenvironment{clai}{\begin{claim}}{\end{claim}}
\newenvironment{defi}{\begin{definition}}{\end{definition}}
\newenvironment{defn}{\begin{definition}}{\end{definition}}
\newenvironment{assu}{\begin{assumption}}{\end{assumption}}
\newenvironment{rema}{\begin{remark}}{\end{remark}}
\newenvironment{rem}{\begin{remark}}{\end{remark}}
\newenvironment{cons}{\begin{construction}}{\end{construction}}
\newenvironment{obse}{\begin{observation}}{\end{observation}}
\newenvironment{fct}{\begin{fact}}{\end{fact}}


\ifnum\abbrevref=0			%Tell cleveref what words to use in front of a reference (abbrevref=0)
	\crefname{assumption}{Assumption}{Assumptions}
	\crefname{construction}{Construction}{Constructions}
	\crefname{corollary}{Corollary}{Corollaries}
	\crefname{conjecture}{Conjecture}{Conjectures}
	\crefname{definition}{Definition}{Definitions}
	\crefname{exmaple}{Example}{Examples}
	\crefname{lemma}{Lemma}{Lemmata}
	\crefname{observation}{Observation}{Observations}
	\crefname{proposition}{Proposition}{Propositions}
	\crefname{remark}{Remark}{Remarks}
	\crefname{theorem}{Theorem}{Theorems}
\else						%Tell cleveref what words to use in front of a reference (abbrevref=1)
	\crefname{assumption}{Ass.}{Ass.}
	\crefname{construction}{Constr.}{Constr.}
	\crefname{corollary}{Cor.}{Cor.}
	\crefname{conjecture}{Conj.}{Conj.}
	\crefname{definition}{Def.}{Def.}
	\crefname{exmaple}{Ex.}{Ex.}
	\crefname{lemma}{Lem.}{Lem.}
	\crefname{observation}{Obs.}{Obs.}
	\crefname{proposition}{Prop.}{Prop.}
	\crefname{remark}{Rem.}{Rem.}
	\crefname{theorem}{Thm.}{Thms.}
\fi

\crefname{claim}{Claim}{Claims}
\crefname{fact}{Fact}{Facts}
\crefname{note}{Note}{Notes}

%Super Mario coin version of \getsr
\def\YYYSMcoin{\mbox{\begin{tikzpicture}[scale=0.0125]
\definecolor{coinbrown}{HTML}{D89E36}\definecolor{coindarkyellow}{HTML}{F8D81E}\definecolor{coinyellow}{HTML}{F8F800}\fill[coinyellow] (3,-1) rectangle (9,9);\fill(0,0) rectangle (1,8);\fill(1,8) rectangle (2,10);\fill(2,10) rectangle (4,11);\fill(4,11) rectangle (8,12);\fill(8,11) rectangle (10,10);\fill(10,10) rectangle (11,8);\fill(11,8) rectangle (12,0);\fill(10,-2) rectangle (11,0);\fill(8,-3) rectangle (10,-2);\fill(4,-4) rectangle (8,-3);\fill(2,-3) rectangle (4,-2);\fill(1,0) rectangle (2,-2);\fill (5,-1) rectangle (7,0);\fill (7,0) rectangle (8,8);\fill[coinbrown] (9,8) rectangle (10,10);\fill[coinbrown] (10,0) rectangle (11,8);\fill[coinbrown] (9,-2) rectangle (10,0);\fill[coinbrown] (8,-2) rectangle (9,-1);\fill[coinbrown] (4,-3) rectangle (8,-2);\fill[coindarkyellow] (2,-2) rectangle (3,8);\fill[coindarkyellow] (3,-2) rectangle (8,-1);\fill[coindarkyellow] (8,-1) rectangle (9,0);\fill[coindarkyellow] (9,0) rectangle (10,8);\fill[coindarkyellow] (8,8) rectangle (9,10);\fill[coindarkyellow] (4,9) rectangle (8,10);\fill[coindarkyellow] (3,8) rectangle (4,9);\fill[coindarkyellow] (5,0) rectangle (7,2);\fill[coindarkyellow] (6,2) rectangle (7,8);\fill[white] (4,0) rectangle (5,8);\fill[white] (5,8) rectangle (7,9);
\end{tikzpicture}}}

%Die version of getsr
\def\YYYdie{\mbox{\begin{tikzpicture}[scale=0.85,x=1em,y=1em,radius=0.09]
\draw[rounded corners=1,line width=.25pt] (0,0) rectangle (1,1);\fill (0.275,0.275) circle;\fill (0.725,0.725) circle;\fill (0.5,0.5) circle;\fill (0.275,0.725) circle;\fill (0.725,0.275) circle;
\end{tikzpicture}}}

\newcommand{\getsr}{
	\ifnum\dieordollar=0
		\mathrel{\vbox{\offinterlineskip\ialign{
			\hfil##\hfil\cr
			\hspace{0.1em}$\scriptscriptstyle\$$\cr
			$\leftarrow$\cr
		}}}
	\fi
	\ifnum\dieordollar=1
		\mathrel{\vbox{\offinterlineskip\ialign{
			\hfil##\hfil\cr
			{\scalebox{0.5}{\hspace{0.4em}\YYYdie}}\cr
			\noalign{\kern0.05ex}
			$\leftarrow$\cr
		}}}
	\fi
	\ifnum\dieordollar=2
		\mathrel{\vbox{\offinterlineskip\ialign{
			\hfil##\hfil\cr
			\hspace{0.1em}$\YYYSMcoin$\cr
			$\leftarrow$\cr
		}}}
	\fi
}

\newcommand{\testequal}{
	\mathrel{\vbox{\offinterlineskip\ialign{
			\hfil##\hfil\cr
			\hspace{0.1em}$\scriptscriptstyle?$\cr
			$\leftarrow$\cr
		}}}
}
\newcommand{\checkfornotes}{
	\ifnum\notesindocument=1
		\ifnum\LNCSpreview=1
			\begin{textblock}{1}[0.5,0](0,0.25)
		\else
			\begin{textblock}{1}[0.5,0](0,0.85)
		\fi
		\centering
		\textcolor{red}{\large \textbf{There are still unresolved comments in this document.}}
		\end{textblock}
	\fi
}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%     SOME COMMANDS FOR FONTS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\varfont}[1]{\mathit{#1}}
\newcommand{\algfont}[1]{\mathsf{#1}}
\newcommand{\termfont}[1]{\mathsf{#1}}
\newcommand{\orfont}[1]{{\ensuremath{\textsc{#1}}}\xspace}
\newcommand{\eventfont}[1]{\mathsf{#1}}
\newcommand{\mat}[1]{\vec{#1}}


==> chapters/construction-efficiency-more-general.tex <==

\clearpage
\subsection{Efficiency}
\bwnote{This section uses some random variables. At some point we need to make sure that we don't already have other names for those in other sections; also, I have used virtual nodes in some parts, and not in others. Maybe remove $K$ entirely from this section?}
We now discuss the efficiency of our protocol.
Note that while the number of adversarial parties has no impact on the robustness of our protocol, efficiency depends on the total number of parties, and therefore on the number of adversarial parties.

\superparagraph{Latency and Round Complexity.}
When an honest party calls, $\iGet$, the latency is at most $3$. Precisely, a call to $\iGet$ made at time $\tau$ returns either a valid $x$ at time $\tau+2$ or $\bot$ at time $\tau+3$.
For interface $\iStore$, the user calling $\iStore$ at $\tau$ does not expect a response and the call returns immediately.
By the end of round $\tau+2$, all messages caused by this call have been received.
For $\iJoin$ called at time $\tau$, the call terminates at $\tau+2+\SubnetDelay$. Synchronization of data may take longer, but we emphasize that as soon as the call is terminated, the party can already participate in the protocol via $\iGet$ and $\iStore$.

\superparagraph{Data Per Node.}
We first examine how much data a node needs to store.
For simplicity, assume that exactly one file $(x_1,\dots,x_\FileLength) \in \SymbolSpace^\FileLength$ is stored.
Recall that each party resides in exactly one column and that nodes in a column are responsible for storing $\FileLength/k_2$ symbols.
Therefore, the data storage requirement for each node is $\FileLength/k_2$.
Now, consider a more general setting in which a node runs $K$ virtual nodes (as discussed in \cref{sec:extensions}).
In this case, a naive upper bound for the storage requirement is $K \FileLength / k_2$, as each of the virtual nodes is in one column.
However, it will be likely that some of the virtual nodes are in the same column, which means that the node only has to store the symbols of that column once.
We will now compute the expected number of symbols that a node $\party$ has to store, for a fixed node $\party$ that runs $K$ virtual nodes, with probability taken over the randomness of the random oracle.
Denote the random variable modeling this number of symbols by $\mathsf{NumSymbStored}$, and for each column $c$, let $\mathsf{InCol}^{\party}_c$ denote the event that $\party$ runs a virtual node that is in column $c$. Clearly, we have \[\Pr\left[ \mathsf{InCol}^{\party'}_c \right] = 1-\left(1-\frac{1}{k_2}\right)^K.\]
Then, we get
\begin{align*}
    \Expect{\mathsf{NumSymbStored}} &=\frac{\FileLength}{k_2} \cdot \sum_{c \in [k_2]} \Pr\left[ \mathsf{InCol}^{\party}_c \right] \\&= \frac{\FileLength}{k_2} \cdot \sum_{c \in [k_2]} \left(1-\left(1-\frac{1}{k_2}\right)^K\right) = \FileLength\cdot \left(1-\left(1-\frac{1}{k_2}\right)^K\right).
\end{align*}

\superparagraph{Connections Per Node.}
Now, let us consider how many connections to peers a node needs to keep.
We consider a fixed point in time $\tau$ and assume that there are $n$ parties in total.
We also assume that each node runs $K$ virtual nodes. Our goal is to derive a bound for the expected number of connections that a fixed node $\party$ has to maintain, taking the randomness over the random oracle. We also assume that $\party$ is not a bootstrap node ($\AuxRole = 0$).
For a column $c$ (resp. row $r$) let $\mathsf{InCol}^{\party'}_c$ (resp. $\mathsf{InRow}^{\party'}_r$) denote the event that a node $\party'$ is in column $c$ (resp. row $r$).
Let $\mathsf{Peers}$ denote the random variable modeling the set of peers that our fixed party $\party$ has. For each column $c$ (resp. row $r$) in which $\party$ resides, let $\mathsf{ColConns}_c$ (resp. $\mathsf{RowConns}_r$) denote the set of pairs $(\party',c)$ such that $\party'$ is also in $c$ (resp. $r$). If $\party$ is not in $c$ (resp. $r$), we define these sets to be empty.
Fix a row $r$, a column, and a party $\party'$. Then, we have \[
    \Pr\left[ \mathsf{InRow}^{\party'}_r \right] = 1-\left(1-\frac{1}{k_1}\right)^K \text{ and } \Pr\left[ \mathsf{InCol}^{\party'}_c \right] = 1-\left(1-\frac{1}{k_2}\right)^K.
\]
Another observation is that
        \[
            \mathsf{Peers} \subseteq \left(\bigcup_{r \in [k_1]} \mathsf{RowConns}_r \right)  \cup \left(\bigcup_{c \in [k_2]} \mathsf{ColConns}_c \right).
        \]
Now, we look at the expectation:
        \begin{align*}
            \Expect{|\mathsf{Peers}|} \leq \left(\sum_{r \in [k_1]} \Expect{|\mathsf{RowConns}_r|}\right) + \left(\sum_{c \in [k_2]} \Expect{|\mathsf{ColConns}_c|}\right).
        \end{align*}
        We fix a row $r$ and consider the expectation of $|\mathsf{RowConns}_r|$. The argument for columns will be similar.
        We have \begin{align*}
            \Expect{|\mathsf{RowConns}_r|} = \Pr\left[ \mathsf{InRow}^{\party}_r \right]\cdot \Expect{|\mathsf{RowConns}_r| \mid \mathsf{InRow}^{\party}_r} + 0.
         \end{align*}
         Further, we have \begin{align*}
            \Expect{|\mathsf{RowConns}_r| \mid \mathsf{InRow}^{\party}_r} = \sum_{\party' \neq \party} \Pr\left[ \mathsf{InRow}^{\party'}_r \right] = (n-1) \left(1-\left(1-\frac{1}{k_1}\right)^K\right).
        \end{align*}
        So, we get \begin{align*}
            \Expect{|\mathsf{Peers}|} \leq k_1 (n-1) \left(1-\left(1-\frac{1}{k_1}\right)^K\right)^2 + k_2 (n-1) \left(1-\left(1-\frac{1}{k_2}\right)^K\right)^2.
        \end{align*}
        For the special case of $K = 1$, this becomes  \begin{align*}
            \Expect{|\mathsf{Peers}|} \leq \frac{n-1}{k_1} + \frac{n-1}{k_2}.
        \end{align*}

\superparagraph{Communication Complexity.}
For communication complexity, we consider the expected total communication that is caused by honest parties calling interfaces $\iGet$ and $\iStore$.
For simplicity, we only consider the setting $K = 1$.
We do only count the outgoing data of honest parties, as one can never limit the amount of data that dishonest parties send.
For simplicity, we denote the maximum size of a single message (with prefix $\msgGet,\msgGetRsp$ or $\msgStore$, $\msgStoreFwd$) by $L_{\mathsf{msg}}$.
Note that $L_{\mathsf{msg}}$ depends on the parameters $|\HandleSpace|$, $\FileLength$, and $|\SymbolSpace|$.

First, consider an honest party calling $\iGet(h,i)$.
Recall that this party identifies a cell $(r,c)$, where column $c$ is responsible for storing the $i$th symbol, and then sends a $\msgGet$-message to all nodes in that cell. The nodes respond with a $\msgGetRsp$-message. We use $|\cdot|$ to denote the length of strings, and denote by $\mathsf{NumNodesInCell}_{r,c}$ (resp. $\mathsf{NumHonNodesInCell}_{r,c}$) the random variable modeling the number of nodes (resp. honest nodes) in cell $(r,c)$.
Then, the expected (over the choice of the random oracle) communication complexity is
\begin{align*}
    \Expect{\mathsf{NumNodesInCell}_{r,c}} \cdot L_{\mathsf{msg}} + \Expect{\mathsf{NumHonNodesInCell}_{r,c}} \cdot L_{\mathsf{msg}} = \left(\frac{n}{k_1k_2} + \frac{\NumberOfHonestParties}{k_1k_2}\right)\cdot L_{\mathsf{msg}}.
\end{align*}
Treating $L_{\mathsf{msg}}$ as constant, this grows asymptotically as $\Theta(n/(k_1k_2))$.
\bwnote{TODO. Apply relation between $n$ and $k_1, k_2$ from robustness analysis.}

Next, we consider an honest party calling $\iStore(h,i,x)$.
The party again identifies all parties in an appropriate cell $(r,c)$ and then sends a $\msgStore$-message. All parties in the cell then send $\msgStoreFwd$-messages to all parties in column $c$.
Denoting the number of parties in column $c$ by ${\mathsf{NumNodesInCol}_{c}}$, the following random variable models the communication complexity:
\begin{align*}
    &\mathsf{NumNodesInCell}_{r,c} \cdot L_{\mathsf{msg}} +{\mathsf{NumHonNodesInCell}_{r,c}} \cdot  \mathsf{NumNodesInCol}_{c} \cdot L_{\mathsf{msg}}.
\end{align*}
To get an upper bound on the expectation, we use \cref{cor:expectationofproduct} with $Y = \mathsf{NumHonNodesInCell}_{r,c}$, $X = \mathsf{NumNodesInCol}_{c}$, and $p = 1/k_2$. Then, as soon as $n \geq 3 k_2 \ln k_2$, the expected communication becomes
\begin{align*}
    \left(\frac{n}{k_1k_2} + \frac{3\NumberOfHonestParties n }{k_1k_2^2} \right)\cdot L_{\mathsf{msg}}.
\end{align*}
\bwnote{TODO. Apply relation between $n$ and $k_1, k_2$ from robustness analysis.}


\bwnote{discuss amplification vectors?}

==> chapters/definitions-comparison_to_dhts.tex <==
\subsection{Comparison to Distributed Hash Tables}
\bwnote{Need to check if this is still all correct once we fixed the final final definition}
In many ways, the object that we construct is similar to distributed hash tables, a well studied object in distributed computing.
Therefore, we want to compare our robust distributed arrays with distributed hash tables here.

\superparagraph{Distributed Hash Tables.}
A \emph{hash table} is a classical data structure that realizes a \emph{key-value store}.
Namely, for a large universe of keys $\UUU$ and a domain $\VVV$ of values, it can dynamically and efficiently maintain a partial mapping $T\colon\UUU \rightarrow \VVV$.
Concretely, it supports an \emph{insert} operation, which given a key $k \in \UUU$ and a value $v \in \VVV$ sets $T(k) := v$, and a \emph{query} operation which given a key $k \in \UUU$ return $T(k) \in \VVV \cup \{\bot\}$.
A \emph{distributed hash table} is a key-value store that is maintained in a distributed fashion: the keys are (potentially redundantly) stored across numerous nodes, and it specifies network protocols to insert or query key-value pairs efficiently (e.g., by contacting only a few nodes). Importantly, such distributed hash tables function when the set of nodes constantly changes and nodes only have a local view of the network topology.
Prominent examples of distributed hash tables are Pastry~\cite{Pastry}, Chord~\cite{Chord}, and Kademlia~\cite{Kademlia}.

\superparagraph{Flat Key Space vs. Indices.}
In a distributed hash table, one can query and insert key-value pairs with keys from an arbitrarily large universe $\UUU$. Typically, there is no structural requirement on $\UUU$, e.g., $\UUU = \bool^{256}$ is possible, and the set of actual keys that will ever be inserted is only a small subset of $\UUU$.
In contrast, in robust distributed arrays, parties query indices $i \in [\FileLength]$ which we could view as keys: keys are always reasonably small integers.

\superparagraph{Robustness.}
Most distributed hash tables are not analyzed with respect to adversarial behavior, with some exceptions~\cite{DBLP:conf/osdi/CastroDGRW02,DBLP:conf/iptps/NaorW03,DBLP:conf/esa/FiatSY05,DBLP:conf/icalp/AwerbuchS04,STOC:Scheideler05,DBLP:conf/spaa/AwerbuchS06,DBLP:conf/iptps/AwerbuchS07,DBLP:journals/ton/YoungKGK13,DBLP:conf/podc/GuerraouiHK13}.
%
However, even these exceptions do not have fully formal definitions of what robustness in presence of an adversary would mean.
Our robust distributed array definition instead makes this very explicit.


==> chapters/intro-contributions.tex <==
\subsection{Our Contributions}
\bwnote{The following are just notes. Should also say why other solutions, e.g., based on DHTs, are not useful for us (polylog overhead, honest majority for the robust ones).}
Our contributions:
\begin{itemize}
    \item A formal definition of what we call \emph{Robust Distributed Arrays (RDAs)}, which is motivated by the requirements of p2p networking in DAS. RDAs can be used to implement the networking layer of DAS.
    \item A simple and efficient RDA construction with the following properties: \begin{itemize}
        \item \emph{Provable Robustness.} We rigorously prove robustness according to our definition.
        \item \emph{Minimal Honesty Assumption.} Our proof tolerates a dishonest majority of participants. Concretely, we only assume that a sufficiently large \emph{absolute} number $N$ of honest parties is online in sufficiently large time intervals.
        \item \emph{Minimal Latency.} The operations supported by our protocol (store and get) incur a small (i.e., constant-round) latency.
        \item \emph{Efficiency Tradeoff.} Our construction implements an efficient tradeoff between the data storage requirements per node, their bandwidth, and $N$.
    \end{itemize}
\end{itemize}

==> chapters/intro-outline.tex <==
\subsection{Organization of this Paper}
In \cref{sec:prelims}, we introduce some notation and our model, including network and adversarial model.
In \cref{sec:rda}, we give our definition of robust distributed arrays and explain how it relates to data availability sampling.
We present and analyze our construction in \cref{sec:construction}.
This section also contains an informal overview of our construction and the definition of an abstract subprotocol, namely, (robust) subnet discovery protocols.
We give an example implementation of such a protocol in \cref{sec:appendix:simplesubnetprotocol}. We discuss several extensions of our protocol that are useful in practice in \cref{sec:extensions}, give benchmarks in \cref{sec:benches}, and discuss related work more extensively in \cref{sec:relwork}.


==> titlepage.tex <==
% Just in case somebody should ever dare to touch those lines: Here's an explanation for provideauthors. The other commands provide... are constructed analogously.
%Please study the code block in main.tex that defines createauthor, createinstitute, first.
%Again, createinstitute is defined similarly to createauthor. On every call of createauthor{}{}{}{} a counter (starting at 0) is increased by 1 and the author's information is stored as a new command that looks like #name, #institute, ... for # in the naturals.
%Back to these commands: Provideauthors is defined recursively and adds 1name, 2name, 3name, ... to the authors as long as there are authors. All the \csname\endcsname commands are used to tell LaTeX to interpret it's content as a string and then consider it as a command. Otherwise, LaTeX won't understand commands like \1name, ....

\newcount\authorcounter
\newcommand{\provideauthors}{%
		\ifnum\authorcounter<\theauthorcount%if there is at least one more author to come
			\csname\the\authorcounter name\endcsname% output the current authorname 
			\expandafter\ifx\csname\the\authorcounter thanks\endcsname\empty%if thanks are not empty for that author, 
			\else
				\thanks{\csname\the\authorcounter thanks\endcsname}% outputs thanks
			\fi%
			\inst{\csname\the\authorcounter institute\endcsname} % add institute number to author.
			\and %places a , between authors and an ", and" between the last two (only for lncs)
			\global\advance\authorcounter by 1 % increase the counter that keeps track of how many authors have been placed
			\provideauthors%run provideauthors again
		\else% i.e. the current author is the last one. (Same code as above, but no \and after placing the author
			\csname\the\authorcounter name\endcsname % output the current authorname
			\expandafter\ifx\csname\the\authorcounter thanks\endcsname\empty %if thanks are not empty for that author, 
			\else
				\thanks{\csname\the\authorcounter thanks\endcsname} % outputs thanks
			\fi%
			\inst{\csname\the\authorcounter institute\endcsname} % add institute number to author.
		\fi
}

\def\atleastoneauthorplaced{0}
\newcommand{\providerunning}{%
	\ifnum\authorcounter<\theauthorcount%
		\expandafter\ifx\csname\the\authorcounter running\endcsname\empty
		\else
			\ifnum\authorcounter>1
				\ifnum\atleastoneauthorplaced=1
					\and%
				\fi
			\fi
			\csname\the\authorcounter running\endcsname
			\def\atleastoneauthorplaced{1}
		\fi
		\global\advance\authorcounter by 1
		\providerunning%
	\else%
		\expandafter\ifx\csname\the\authorcounter running\endcsname\empty
		\else
			\ifnum\authorcounter>1
				\ifnum\atleastoneauthorplaced=1
					\and%
				\fi
			\fi
			\csname\the\authorcounter running\endcsname
		\fi
	\fi
}

\newcount\institutecounter

\newcommand{\provideinstitutes}{%
	\ifnum\institutecounter<\theinstitutecount%
		\ifnum\llncs=0
			$^{\csname\the\institutecounter number\endcsname}$
		\fi
		\csname\the\institutecounter instname\endcsname
		
		\email{
			\ifx\contactmail\empty
				\csname\the\institutecounter mail\endcsname
			\else
				\href{mailto:\contactmail}{\csname\the\institutecounter mail\endcsname}
			\fi
		}
		
		\and%
			\global\advance\institutecounter by 1
		\provideinstitutes%
	\else%
		\ifnum\llncs=0
			\ifcsname 1name\endcsname
				$^{\csname\the\institutecounter number\endcsname}$
			\fi
		\fi
		\csname\the\institutecounter instname\endcsname
		
		\email{
			\ifx\contactmail\empty
				\csname\the\institutecounter mail\endcsname
			\else
				\href{mailto:\contactmail}{\csname\the\institutecounter mail\endcsname}
			\fi
		}
	\fi
}

\title{
	\ifnum\stuffedtitlepage=1
		\ifnum\llncs=1
			\vspace*{-7ex}
		\else
		\vspace*{-3ex}
		\fi
		\textbf{\titletext}
		\ifnum\llncs=1
			\vspace*{-2ex}
		\else
			\vspace*{-1ex}
		\fi
	\else
		\textbf{\titletext}
	\fi
}
\ifnum\anonymous=1
	\author{}
\else
	\ifnum\llncs=0
		\newcommand{\inst}[1]{{
			\ifcsname 1name\endcsname
				$^{#1}$
			\fi
			}}
	\fi
	\ifcsname 1name\endcsname
		\author{
			\global\authorcounter 1
			\provideauthors
		}
	\fi
\fi

\ifnum\llncs=1
	\titlerunning{\runningtitle}
	\ifnum\anonymous=1
		\institute{}
		\authorrunning{}
	\else
		\ifcsname 1instname\endcsname{
			\institute{
				\global\institutecounter 1
				\provideinstitutes
			}
		\fi
		\ifcsname 1name\endcsname{
			\authorrunning{
				\global \authorcounter 1
				\providerunning
			}
		\fi
	\fi
\fi
\maketitle
\ifnum\stuffedtitlepage=1
	\ifnum\llncs=0
		\vspace{-4ex}
	\fi
\fi

\ifnum\llncs=0
	\ifnum\anonymous=0
		\newcommand{\email}[1]{
			\texttt{
				\ifx\contactmail\empty
					#1
				\else
					\href{mailto:\contactmail}{#1}
				\fi
			}
		}
		\newcommand{\and}{}
		\ifnum\stuffedtitlepage=1
			\ifnum\llncs=0
				\vspace{-2ex}
			\fi
		\fi
		\begin{small}
			\begin{center}
				\global \institutecounter 1
				\provideinstitutes
			\end{center}
		\end{small}
	\fi
\fi

\ifnum\stuffedtitlepage=1
	\ifnum\llncs=1
		\vspace*{-4ex}
	\else
		\vspace*{-2ex}
	\fi
\fi

\begin{abstract}
	\abstracttext
\end{abstract}
\ifnum\stuffedtitlepage=1
	\ifnum\llncs=1
		\vspace*{-2ex}
	\fi
\fi

\ifnum\llncs=0
	\vspace{1ex}
\fi

\ifx\choosepubinfo\empty\else
	\ifnum\choosepubinfo=1
	\def\pubinfo{\small
			\noindent \copyright\ IACR 
			\ifx\pubinfoYEAR\empty \textcolor{red}{year missing}\else \pubinfoYEAR\fi.
			This article is a minor revision of the version published by Springer-Verlag in the proceedings of \ifx\pubinfoCONFERENCE\empty \textcolor{red}{conference missing}\else \pubinfoCONFERENCE\fi, eventually available at \url{http://link.springer.com}
	}
	\fi
	
	\ifnum\choosepubinfo=2
		\def\pubinfo{\small
			\noindent \copyright\ IACR 
			\ifx\pubinfoYEAR\empty \textcolor{red}{year missing}\else \pubinfoYEAR\fi.
			This article is the final version submitted by the author(s) to the IACR and to Springer-Verlag on
			\ifx\pubinfoSUBMISSIONDATE\empty \textcolor{red}{submission date missing}\else \pubinfoSUBMISSIONDATE\fi.
			The version published by Springer-Verlag is available at
			\ifx\pubinfoDOI\empty \textcolor{red}{DOI missing}\else \pubinfoDOI\fi.
		}
	\fi
	
	\ifnum\choosepubinfo=3
		\def\pubinfo{\small
			\noindent \copyright\ IACR
			\ifx\pubinfoYEAR\empty \textcolor{red}{year missing}\else \pubinfoYEAR\fi.
			This article is a minor revision of the version published by Springer-Verlag available at
			\ifx\pubinfoDOI\empty \textcolor{red}{DOI missing}\else \pubinfoDOI\fi.
		}
	\fi
	
	\ifnum\choosepubinfo=4
		\def\pubinfo{\small
			\noindent This article is based on an earlier article:
			\ifx\pubinfoBIBDATA\empty \textcolor{red}{bibliographic data missing}\else \pubinfoBIBDATA\fi,
			\copyright\ IACR
			\ifx\pubinfoYEAR\empty \textcolor{red}{year missing}\else \pubinfoYEAR\fi,
			\ifx\pubinfoDOI\empty \textcolor{red}{DOI missing}\else \pubinfoDOI\fi.
		}
	\fi
	
	\ifnum\choosepubinfo=5
			\def\pubinfo{\small
				\noindent \pubinfoindividual
			}
		\fi
\fi

\textblockorigin{0.5\paperwidth}{0.9\paperheight}
\setlength{\TPHorizModule}{\textwidth}

\newlength{\pubinfolength}
\ifx\choosepubinfo\empty\else
	\ifnum\choosepubinfo=0
	\else
		\settowidth{\pubinfolength}{\pubinfo}
		\begin{textblock}{1}[0.5,0](0,.25)
			 \ifnum\pubinfolength<\textwidth
				\centering
			\fi
			\pubinfo
		\end{textblock}
	\fi
\fi
\thispagestyle{empty}
